Finding Cryptocurrency Attack Indicators Using Temporal Logic and Darkweb Data

With the recent prevalence of darkweb/deepweb (D2web) sites specializing in the trade of exploit kits and malware, malicious actors have easy-access to a wide-range of tools that can empower their offensive capability. In this study, we apply concepts from causal reasoning, itemset mining, and logic programming on historical cryptocurrency-related cyber incidents with intelligence collected from over 400 D2web hacker forums. Our goal was to find indicators of cyber threats targeting cryptocurrency traders and exchange platforms from hacker activity. Our approach found interesting activities that, when observed together in the D2web, subsequent cryptocurrency-related incidents are at least twice as likely to occur than they would if no activity was observed. We also present an algorithmic extension to a previously-introduced algorithm called APT-Extract that allows to model new semantic structures that are specific to our application.

==> conclusion.tex <==

\section{Related Work.}

To the best of our knowledge, this paper is the first to present an AI-based approach that associates threat actor activity in the D2web with real-world and large-scale attacks to cryptocurrencies technologies. Being said, there exists a large volume of research that leveraged signals from the D2web or social network platforms to predict future cyber threats or detect ongoing threats~\cite{ Almukaynizi2017proactive,Tavabi2018iaai,sapienza2017early, almukaynizi2017predicting}. However, none of those studies focused on the predictions of events related to the cryptocurrency platforms, a problem we tackle in this paper. The work related to cryptocurrencies has mostly focused on the security aspects related to the underlying blockchain framework~\cite{lin2017survey}, or on forecasting the price movements of certain cryptocurrencies~\cite{indera2017non, mcnally2018predicting}. More related to our approach, but not focused on cryptocurrency, Stanton et al.~\cite{stanton2015mining} used the formalism of APT-logic to correlate military activity surrounding ISIS in Syria and Iraq with the forces against it and presented interesting relationships. 




\section{Conclusion}
\vspace{1em}
This study presents an approach that combines concepts from causal reasoning, itemset mining, and logic programming. This approach identifies indicators of cyber threats to cryptocurrency traders and exchange platforms from hacker activity in D2web. We show interesting correlations from the APT rules. In the future, we plan to use the approach with other sources such as social media platforms. Additionally, we plan to incorporate the learned rules into an alert system that generates and visualizes warnings.

==> exp.tex <==
\vspace{1em}
\vspace{1em}

\section{Experiments and Analysis}
\vspace{1em}
This section presents the results of a series of experiments to illustrate the viability of our approach. In particular, we show: (1) the rules that are preconditioned on itemsets tend to have higher correlations with future incidents than the rules that are preconditioned on single atoms, and (2) the performance of our approach change leanierly when $\Delta t_{act}$ is extended. We also show the change in the number of rules that were identified as being ``useful" (i.e., having a positive increase in probability and with decent support count) when other variables are varied. 

%TODO: exp1



\noindent\textbf{Itemset Rules vs. Atomic Rules.} Interestingly, the \textit{efr}'s whose precondition is itemsets have notably higher probabilities than those whose precondition is single tags. It is evident (from Figure~\ref{prob}) that the usage of the Apriori algorithm  with APT-logic added considerable value to the generated rules. 

\begin{figure}[!h]
	\centering
	\includegraphics[scale=0.12,keepaspectratio]{./images/box_plot_probability.pdf}
	\caption{Box plot showing precondition type (itemset-rules, single-atom-rules) vs. probability.}
	\label{prob}
\end{figure}
\vspace{1em}

Although the single atoms that are used as preconditions of the generated rules may not be in any of the frequent itemsets, the single-atom-rules have on average higher support than the frequent-itemset-rules as depicted in Figure~\ref{support}. This suggests that an atom of an itemset does not necessarily occur when another atom in that same itemset is observed i.e., less co-occurrence. 

\begin{figure}[!h]
	\centering
	\includegraphics[scale=0.12,keepaspectratio]{./images/box_plot_support.pdf}
	\caption{Box plot showing precondition type (itemset-rules, single-atom-rules) vs. support}
	\label{support}
\end{figure}
\vspace{1em}





%TODO: exp2

\noindent\textbf{Run-time Analysis.} Figure \ref{fig3} shows that when the length $\Delta t_{act}$ increases, the time taken for \textit{APT-EXTRACT} to generate rules increases linearly, because the number of time points for which \textit{APT-EXTRACT} needs to check the satisfaction of the consequence increases. This shows that our approach is flexible to applications where the user wants to extend the length of time units are which \textit{efr}'s are computed. However, we shall note that the Apriori algorithm runs in exponential time, and for all analysis in this study, we restrict the number of items to 2 in each itemset, and we don not introduce more types of atoms (tags).\smallskip


\begin{figure}[!h]
	\centering
	\includegraphics[scale=1.4,keepaspectratio]{./images/3_time_graph_1.pdf}
	\caption{Time taken to generate rules when varying $\Delta t_{act}$.}
	\label{fig3}
\end{figure}
\vspace{1em}






%TODO: exp3


\noindent\textbf{Varying the Variables.} We run series of experiments to show the relationship between the number of produced rules that have probabilities exceeding the probability of a null rule when we vary the values of certain variables like $\Delta t_{con}$, type of cryptocurrency, and the value of $\Delta t_{act}$. Figure \ref{fig1} shows that there are less significant rules with the 1-day-sliding-window run as compared to the 5-day-sliding-window run. This is mainly because when $\Delta t_{con}$ rises, it gives more time-window between related D2web activities to occur together and form frequent itemsets. This makes the number of possible preconditions increase, resulting in more significant \textit{efr}'s. The count of significant rules does not seem to correlate with value of $\Delta t_{act}$; however, relative likelihood starts to drop after $\Delta t_{act}$ reaches certain value (e.g., at 7-10 time-points for Bitcoin, 10-15 time-points for Ethereum, and 8-12 for general cryptocurrencies; depending also on $\Delta t_{con}$). This drop is due to the fact that the probability of a null rule also increases as $\Delta t_{act}$ raises.\smallskip %Although the probability of the null rule increases when $\Delta t$ is raising, larger $\Delta t$ allows for more time for a major cryptocurrencies-related incident to occur after an activity with little correlation with those attacks is observed. However, this is not always the case. The type of cryptocurrencies plays little role related to the count of significant rules. This might be an indicator that rules for Bitcoin-related attacks may be useful to predict Ethereum-related incidents, and vise versa. 

\begin{figure}[!h]
	\centering
	\includegraphics[scale=1.4,keepaspectratio]{./images/1_count_graph_1.pdf}
	\caption{The number of rules produced for each cryptocurrency when varying $\Delta t_{con}$ and $\Delta t_{act}$.}
	\label{fig1}
\end{figure}


==> intro.tex <==
\vspace{1em}
\section{Introduction and Dataset}
\vspace{1em}
Cryptocurrencies are digital currencies that mostly use the blockchain concept to record transactions. Perhaps the most well-known one is Bitcoin. Threats to cryptocurrencies by nation state actors has received recent attention as nation states may seek to harm trust and value of such currencies or that they may perceive the cryptocurrency as a national security threat~\cite{rand2015}. However, this has not stopped the continuously growing demand for cryptocurrencies and their exchange platforms\footnote{https://news.bitcoin.com/bitcoin-numbers-21-statistics-reveal-growing-demand-cryptocurrency}, nor has it stopped the growing of their adoption across businesses\footnote{https://cointelegraph.com/news/bitcoin-adoption-by-businesses-in-2017}. For example, it was estimated that the market capitalization of cryptocurrencies has exceeded 400 billion dollars, after peaking at over 700 billion dollars\footnote{https://cointelegraph.com/news/combined-crypto-market-capitalization-races-past-800-bln.}.

With the high reliance on technology, increasing adoption from businesses and traders, and due to the inherent anonymity associated with transactions and wallet owners, malicious threat actors (including hackers and scammers) aiming for financial gain have been highly motivated to hack and scam to gain control over cryptocurrency wallets and perform transactions. 

In this research effort, we have encoded and recorded over 50 major incidents of cyberattacks and scam campaigns targeting multiple cryptocurrencies and traders\footnote{These incidents were extracted from various IT security repositories including https://www.hackmageddon.com, https://www.cryptoaware.org/resources/notable-cryptocurrency-hacks, https://www.livecoinwatch.com, and others.}. A few examples are reported in Table~\ref{1}. We also queried postings from over 400 hacker forums in the D2web using an API that is commercially provided by a threat intelligence firm\footnote{Cyber Reconnaissance, Inc. (CYR3CON), https://www.cyr3con.ai.}. The database is collected from D2web sites that were identified to be serving hacking-related content. Each identified site is regularly scraped using customized lightweight crawlers and parsers. Before passing to the API, irrelevant postings (e.g., related to drugs or weapons) are filtered by machine learning models that are highly accurate (the data collection system was originally introduced in~\cite{Nunes:2016}). Using both databases, we mine for sequential patterns to identify indicators of attacks from the D2web database, which can then be monitored to reason about risks that are likely to occur in the future. Specifically, we found that when certain D2web activities are observed together; subsequent cryptocurrency-related incidents are at least twice as likely to occur than they would if no activity was observed, and significantly more likely to occur than when individual activity is observed.
%, especially, with the lack of explicit discussions about those targets prior to the incidents (e.g., discussions referencing certain attacks or indicating what will be the target and when the attack will take place), which we found to be the case with D2web content. 

\begin{table}[!h]
	\caption{Example attacks}
	\vspace{-1em}
	\label{1}
	\begin{center}
		\begin{tabular}{|l|c|c|}
			\hline
			\bf{Name of Attack} & \bf{Targeted Currency} & \bf{Estimated Loss (in USD)}\\
			\hline
			{Mt Gox Hack } & {Bitcoin } & {450 Millions }\\
			\hline
			{NiceHash Hack } & {Bitcoin } & {62 Millions }\\
			\hline
			{Parity Wallet Hacks } & {Ethereum } & {160 Millions }\\
			\hline
			{Tether Token Hack } & {Tether } & {30 Millions }\\
			\hline
		\end{tabular}

	\end{center}
\end{table} 
\vspace{1em}

To learn such patterns, we sought to derive temporal logic rules of the form ``A cryptocurrency \textit{G} will be targeted by hackers/scammers with a probability \textit{p} within $\Delta t_{act}$ time units after itemset \textit{F} is observed on the D2web within $\Delta t_{con}$ time units". To do so, we combine concepts from logic programming (in particular, the concepts of existential frequent rules (\textit{efr}) from APT logic~\cite{Shakarian:2011, Shakarian:2012}) with frequent itemset mining~\cite{han2000mining} and temporal causal reasoning~\cite{kleinberg2009temporal}. Table~\ref{2} shows some of the interesting \textit{efr}'s obtained from the algorithm. 



\begin{table*}
	\centering
	\caption{Example of ersignificant rules}
	\label{2}
	\renewcommand{\arraystretch}{1.5}
	\begin{tabular}{|m{6cm}|c|m{6cm}|}
		\hline 
		\textbf{Rule} & \textbf{\%increase in likelihood of occurrence} & \textbf{Description} 
		\\ \hline 
		 \textit{Mentioned(Coinbase, financial, 10)} $\wedge $    \textit{Mentioned(Gmail, software, 13)}  $ \overset{efr}{\rightlsquigarrow}$
		 	 ~~~~~~~~~~~\textit{Attacked(general, \$175,774,960)}: [21, 0.94, 5]
		& 201\% & When ``Coinbase" as a financial tag and ``Gmail" as a software tag are mentioned more then 10 and 13 times, respectively, within any window of 5 days, there is a 94\% chance that a cryptocurrency-related incident with an average loss of \$174,774,960 would happen in the next $21$ days. This is 201\% more likely to occur than the chance of occurring in any sequence of 21 days. 
		\\%[-1em]
		\hline  
		\textit{Mentioned(Mastercard, financial, 17)} $\wedge $  ~~~~~~~~~~~\textit{Mentioned(Whatsapp, software, 28)} $\overset{efr}{\rightlsquigarrow} $  \textit{Attacked(Bitcoin, \$ 9,803,571)}: [7, 0.32, 5] 
		& 4.50\% &  Similarly, when ``Mastercard" as a financial tag and ``Whatsapp" as a software tag are mentioned more then 17 and 28 times, respectively, there is a 32\% chance of a Bitcoin attack/scam event with an average loss of \$9,803,571 would happen in the next 7 days. However, this rule has a very low support\textemdash low support rules are not very reliable.\\ 
		\hline 
				\textit{Mentioned(SQL, software, 19)} $ \wedge $  ~~~~~~~~~~~~~~~\ ~~~~~~~~~~~\textit{Mentioned(Windows Registry, software, 19)} $\overset{efr}{\rightlsquigarrow} $ \textit{Attacked(Ethereum, \$3,989,215)}: [21, 0.39, 5] 
		&2.06\% &  When ``SQL" as a software tag and ``Windows Registry" as a software tag are mentioned more then 19 times, there is a 39\% chance that a Ethereum event with an average loss of \$3,989,215 would happen in the next 21 days, 206\% increase in likelihood of occurrence. \\ 
		\hline 
	\end{tabular} 
\vspace{1em}

\end{table*}





%\begin{table*}[h]
%	\begin{tabular}[l]{|p{7cm}|c|p{7.5cm}|}
%		\hline
%		\textbf{Formula} & \textbf{Relative likelihood} & \textbf{Description}                                                                                                                                                                                                                                                                                                 \\ \hline
%		\multirow{3}{*}{a}                & \multirow{3}{*}{2.01}                         & \multirow{3}{*}{When Coinbase as a financial tag and Gmail as a software tag are mentioned more then 10 and 13 times, respectively, in the D2Web data within any window of 5 days, then there is a 94\% chance that a cryptocurrency-related incident with the average loss of \$174,774,960 would happen in the next $21$ days.}     \\
%		&                                               &                                                                                                                                                                                                                                                                                                                                       \\
%		&                                               &                                                                                                                                                                                                                                                                                                                                       \\ \hline
%		\multirow{3}{*}{a}                & \multirow{3}{*}{4.51}                         & \multirow{3}{*}{When Mastercard as a financial tag and Whatsapp as a software tag are mentioned more then 17 and 28 times, respectively, in the d2Web data then there is a 32\% chance that a Bitcoin event with an average loss of \$9,803,571 would happen in the next $\Delta t=7$ days. However, this rule has very low support.} \\
%		&                                               &                                                                                                                                                                                                                                                                                                                                       \\
%		&                                               &                                                                                                                                                                                                                                                                                                                                       \\ \hline
%		\multirow{3}{*}{a}                & \multirow{3}{*}{2.06}                         & When SQL as a software tag and Windows }                                                         \\
%		&                                               &                                                                                                                                                                                                                                                                                                                                       \\
%		&                                               &                                                                                                                                                                                                                                                                                                                                       \\ \hline
%	\end{tabular}
%\end{table*}


%\begin{table*}
%\begin{tabular}{|l|cl}
%	\hline
%	\textbackslash{}textbf\{Formula\} & \multicolumn{1}{c|}{\textbackslash{}textbf\{Relative likelihood\}} & \multicolumn{1}{l|}{\textbackslash{}textbf\{Description\}}                                                                                                                                                                                                                                                                                \\ \hline
%	\multirow{2}{*}{a}                & \multicolumn{1}{c|}{\multirow{2}{*}{2.01}}                         & \multicolumn{1}{l|}{When Coinbase as a financial tag and Gmail as a software tag are mentioned more then 10 and 13 times, respectively, in the D2Web data within any window of 5 days, then there is a 94\% chance that a cryptocurrency-related incident with the average loss of \$174,774,960 would happen in the next $21$ days.}     \\
%	& \multicolumn{1}{c|}{}                                              &                                                                                                                                                                                                                                                                                                                                           \\ \hline
%	a                                 & \multicolumn{1}{c|}{4.5}                                           & \multicolumn{1}{l|}{When Mastercard as a financial tag and Whatsapp as a software tag are mentioned more then 17 and 28 times, respectively, in the d2Web data then there is a 32\% chance that a Bitcoin event with an average loss of \$9,803,571 would happen in the next $\Delta t=7$ days. However, this rule has very low support.} \\ \hline
%	a                                 & \multicolumn{1}{c|}{2.06}                                          & \multicolumn{1}{l|}{When SQL as a software tag and Windows Registry as a software tag are mentioned more then 19 times each in the d2Web data then there is a 39\% chance that a Ethereum event with an average loss of \$3,989,215 would happen in the next $\Delta t=21$ days.}                                                         \\ \hline
%\end{tabular}
%\end{table*}



==> preliminaries.tex <==
\vspace{1em}
\section{Motivation}
Nation state actors may seek to attack cryptocurrencies for a variety of reasons, to include creating financial instability in certain markets, harming rival currencies, or even financial gain.  Recent analysis~\cite{rand2015} has viewed this problem through established threat-actor tiers~\cite{dsb}.  However, viewed in the larger context of threats to financial infrastructure, this type of activity is expected. There are many examples of attacks against financial institutions associated with nation state activity. For example, concerted effort by Iranian attackers against American banks started in December 2011 and continued through May 2013 are identified to be nation state sponsored\footnote{https://www.reuters.com/article/us-usa-iran-cyber/u-s-indicts-iranians-for-hacking-dozens-of-banks-new-york-dam-idUSKCN0WQ1JF}. With the advent of blockchain-based cryptocurrencies, which are introduced to be ``secure by design", new concerns related to their security have emerged (see~\cite{lin2017survey} for a survey).  Attacks against the infrastructure (i.e., 51\% attacks) as well as implementation (i.e., schemes to obtain wallet credentials) are currently wide-spread~\cite{eyal2018majority}.  As cryptocurrencies become increasingly entwined with traditional banking mechanisms, sophisticated and/or large-scale attacks against the underlying asset (cryptocurrency) can have a ripple effect\textemdash possibly making it a target of choice for a nation state actor. 


\section{Technical Approach}
\vspace{1em}
\subsection{APT-Logic} 
\noindent\textbf{Concepts.} We use the same syntax and semantics that were previously introduced in our work~\cite{Shakarian:2011, Shakarian:2012, stanton2015mining}. Here, we informally review a subset of those concepts. 

A \textit{thread} is a sequence of \textit{worlds} (events). Each world corresponds to a discrete time point. Time points are represented by natural numbers in the range 1, \dots , $t_{max}$. A \textit{formula} $F$ can be any itemset (in this paper, atoms can only be predicates with arities of 2 or 3, e.g., \{\textit{attacked(Bitcoin, \$1,000,000)},\textit{ mentioned(Coinbase, software, 9)}, \textit{mentioned(Gmail, software, 13)}\}). The atoms used in this study are partitioned into two disjoint subsets: condition atoms from D2web activities ($\mathcal{A}_{con}$), and action atoms from the database of observed incidents ($\mathcal{A}_{act}$).\smallskip

\noindent\textbf{Satisfaction.} We say a thread ($Th$) satisfies a formula $F$ at a time-point $t$ (denoted $Th(t) \models F$) if and only if:  $\forall_{a \in F} (Th(t) \models a)$. \smallskip

\noindent\textbf{Rule probability.} The probability is determined based on the fraction of times where a rule $r$ is satisfied from the times where the precondition is satisfied\footnote{If the precondition is not satisfied by \textit{Th} at any time-point, \textit{p} to set to 1.}. \smallskip


\noindent\textbf{Significance.} We determine whether a rule is statistically significant based on relative likelihood, i.e., the percentage increase in likelihood of occurrence when the precondition is observed.\smallskip

% The probability is the fraction of times where a rule $r$ is satisfied from the times where the precondition is satisfied. Finally, the probability of a null rule with regards to a certain consequence is the probability of a rule with $f \equiv \emptyset$ and $g$ of that consequence.\smallskip


\subsection {D2web Activity} 
\noindent\textbf{Tagging.} The D2web API supplies tags with each post. Each tag should belong to one of three categories: financial, software, or general topic tags. The tagging algorithm leverages document similarity techniques on doc2vec representations of posts to assign tags that are most relevant to each post. Our approach uses the count of tags per day, i.e., when a tag is observed with a count that exceeds certain threshold, an atom respective to that condition becomes true. The said threshold is tag-dependent; meaning each tag has a threshold. We determined thresholds based on average and standard deviation of tag mentions per day in the historical data\footnote{An atom becomes true if, on a given day, its respective tag is mentioned more than the average added to (1.5 * standard deviation).}.\smallskip% Figure \ref{fig2} depicts the count of surging tags per month in our dataset for the tags that subsequently produced interesting rules. \smalls	kip

%\begin{algorithm}[ht]
%	\caption{rolling-window}\label{alg:algorithm1}
%	\begin{algorithmic}[1]
%		\Require
%		\Statex If there are multiple lines here, line's number will be wrong.
%		\Statex This error doesn't happen in package \verb|algorithmic|.
%		\Ensure
%		\Statex If I write \verb|\\| here, line's number will be wrong too.
%		\Statex
%		\If{$i = 1 \to n$} \Comment{This line's number should be 1}
%		\State ${\textit{HU}}_{i} \gets {\textit{NGU}}_{i} + {HU}_{i}$ \Comment{Comment}
%		\EndIf
%	\end{algorithmic}
%\end{algorithm}



%\begin{figure}[!h]
%	\centering
%	\includegraphics[scale=0.22,keepaspectratio]{./images/2_mentions_graph.pdf}
%	\caption{Count of surging tags per month in our dataset for the tags that subsequently produced interesting rules.}
%	\label{fig2}
%\end{figure}


\noindent\textbf{Sliding Window.} The current semantic structure of APT-logic does not capture the concept of \textit{efr}'s whose precondition atoms occur in any order within a sequence of $\Delta t_{con}$ time points. However, the \textit{efr}'s we sought to obtain need such semantics. Therefore, we make a new thread $Th'$ that is derived from $Th$ according to Algorithm~\ref{alg1}. Essentially, this algorithm iterates over $Th$ once; at each time point $t$ it assigns $Th'(t)$ the condition atoms that $Th(t_i)$ satisfies for every $t_i$ in the sequence of time-points $t- (\Delta t_{con} - 1)$, \dots, $t$.



 \begin{algorithm}
	\caption{Forward rolling condition atoms}
	\label{alg1}
	\begin{algorithmic}[1]
		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
		\renewcommand{\algorithmicensure}{\textbf{Output:}}
		\Require Thread $Th$, an empty thread $Th'$, length of threads $t_{max}$, condition atoms $\mathcal{A}_{con}$, and length of rolling window $\Delta t_{con}$
		\Ensure  Forward-rolled thread $Th'$
		%\\ \textit{Initialisation} :
		\State $window\_size \gets \Delta t_{con} -1$ 
		%\\ \textit{LOOP Process}
		\For {$t \in \{1, \dots , t_{max}\}$}
		\For {$t_i \in \{max(1, t-window\_size), \dots , t\}$}
		\For {$g \in \{a \in \mathcal{A}_{con} \ where \ Th(t_i) \models a\}$}
		%\STATE statements..
		\State $Assign(Th'(t), g)$  \Comment{assigns $g$ to $Th'(t)$ if $Th'(t) \nvDash g$ }
		\EndFor
		\EndFor

		\EndFor\\
		\Return $Th'$ 
	\end{algorithmic} 
\end{algorithm}
\vspace{1em}

%\begin{equation}
%\small
%\begin{split}
%	\forall_{a \in A, t \in [1, \dots, t_{max}]} &(Th(t) \models a \\ & \rightarrow (\forall_{x \in [t, \dots, min(t + \Delta x, t_{max})]} (Assign(Th'(x), a)))
%\end{split}
%\end{equation}

%Where the function $Assign(Th'(x), a)$ assigns an atom $a$ to the thread $Th'$ at time-point $x$ (i.e., $Th'(x) \models a$). \smallskip

\noindent\textbf{Itemsets.} The preconditions of our \textit{efr}'s are frequent itemsets, obtained from running the Apriori algorithm~\cite{han2000mining}. The input to the Apriori algorithm is a database of transactions\textemdash each world corresponding to a time-point in $Th'$ can be regarded as a transaction. The output is all itemsets that are satisfied by the thread with a frequency exceeding a minimum support\footnote{$min\_support$ is experimentally-determined and set to ($0.13 * t_{max}$).}. We run the Apriori algorithm on $Th'$. The algorithm returns frequent itemsets (denoted $freqItemsets$). Then we make a thread $Th_{itemsets}$ only containing atoms (frequent itemsets) that $Th'$ satisfies at each time point as illustrated in Algorithm~\ref{alg2}.\smallskip





\begin{algorithm}
	\caption{Construct $Th_{itemsets}$ }
	\label{alg2}
	\begin{algorithmic}[1]
		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
		\renewcommand{\algorithmicensure}{\textbf{Output:}}
		\Require Thread $Th$, thread $Th'$, an empty thread $Th_{itemsets}$, length of thread $t_{max}$, $freqItemsets$, and action atoms $\mathcal{A}_{act}$
		\Ensure  $Th_{itemsets}$
		%\\ \textit{Initialisation} :
		%\State $window\_size \gets \Delta t_{con} -1$ 
		%\\ \textit{LOOP Process}
		\For {$t \in \{1, \dots , t_{max}\}$}
		\For {$I \in freqItemsets$}
		
		\If {$I \subseteq Th'(t)$}
		\State $Assign(Th_{itemsets}(t), I)$ 
		\EndIf	
		\EndFor
		\For {$g \in \{a \in \mathcal{A}_{act} \ where \ Th(t) \models a\}$}
		\State $Assign(Th_{itemsets}(t), g)$
		\EndFor
		\EndFor\\
		\Return $Th_{itemsets}$
	\end{algorithmic} 
\end{algorithm}
\vspace{1em}



%\begin{equation}
%\small
%\begin{split}
%\forall_{I} \  \forall_{t} &( I \subseteq Th'(t) \land I \in freqItemsets \land t \in \{1, \dots, t_{max}\})\\ &\implies (Assign(Th_{itemsets}(t), I)))
%\end{split}
%\end{equation}
%
%
%
%\begin{equation}
%\small
%\begin{split}
%\forall_{I \in freqItemsets, t \in [1, \dots, t_{max}]} &( I \subseteq Th'(t) \\ &\rightarrow (Assign(Th_{itemsets}(t), I)))
%\end{split}
%\end{equation}


\noindent\textbf{\textit{efr} Rule-Learning.} We use the algorithm \textit{APT-EXTRACT} to mine for \textit{efr}'s~\cite{Shakarian:2011}. Essentially, \textit{APT-EXTRACT}  produces all rules whose precondition is any of the itemsets that are satisfied by the thread at $n$ or more time points, i.e., $n$ is greater than a minimum (lower bound) support (specified by the argument \textit{SuppLB}~\cite{Shakarian:2011}).\smallskip


==> relwork.tex <==
\section{Related Work.}

%To the best of our knowledge, this paper is the first study that applies inductive reasoning to identify causal relationships and reason about cyber-security events related to specific enterprises. We also extend the framework of \cite{DBLP:journals/corr/abs-1205-2634} and APT-logic with notations and algorithms related to our specific application. However, there exists a large body of related research with studies related to malicious hacking community in D2web, studies and applications of rule-learning methods, and studies that apply machine learning to predict cyber attacks.


%\noindent\textbf{Studies on malicious hacking community on D2web.}.  While hacking community in D2web sites have been widely investigated in the existing literature for applications such as analyzing the economics of D2web forums/markets \cite{motoyama2011analysis,kwon2017crisis,shakarian2016exploring}, recognizing and categorizing D2web hacking-related content \cite{robertson2017darkweb,Nunes:2016,ghosh2017automated}, and identifying future cyber-threats to mitigate risks \cite{Almukaynizi2017proactive,Tavabi2018iaai,sapienza2017early}, none of these studies identify threats related to specific corporate; nor do they identify when in the future the predicted events may occur. In this paper, we use a dataset of enterprise-related external attack events that are detected in the wild, and relate threats to targets and attacks types. We also leverage inductive reasoning to identify the periods in which threats are predicted as well as the volume of predicted attacks, a problem that has not been investigated previously. 

%\noindent\textbf{Application Rule-learning methods security application.}There has been proposed a large body of work on understanding and modeling the behavior of threat actors and reasoning about risk levels in future to aid in implementing strategic defense. While a growing number of papers along this track have focused on applications related to understanding the behaviour of terrorist and insurgent groups \cite{subrahmanian2013indian,Stanton:2015,mannes2008stochastic}, the cyber-security applications have not received much of attention, except in the line of applications of graph-based and attacker/defender game theoretical modeling \cite{robertson2016data,pibil2012game,brown2014addressing}. Our work differs from those papers in the sense that our system is deployed and we use real-world . The contributions in the cyber-security field are many, but the focus is mainly on enhancing intrusion detection and signature-based systems \cite{Mitchell2015,garcia2009anomaly}. Such systems rely solely on the network traffic. While effective in preventing known threats and suspicious behaviour, those systems can rarely aid in the identification of previously unseen risks/behaviours \cite{liao2013intrusion}, and allocating resources accordingly.

